Structure and Dynamics of Magneto-Inertial, Differentially Rotating Laboratory Plasmas

We present a detailed characterization of the structure and evolution of differentially rotating plasmas driven on the MAGPIE pulsed-power generator (1.4 MA peak current, 240 ns rise-time). The experiments were designed to simulate physics relevant to accretion discs and jets on laboratory scales. A cylindrical aluminium wire array Z pinch enclosed by return posts with an overall azimuthal off-set angle was driven to produce ablation plasma flows that propagate inwards in a slightly off-radial trajectory, injecting mass, angular momentum, and confining ram pressure to a rotating plasma column on the axis. However, the plasma is free to expand axially, forming a collimated, differentially rotating axial jet that propagates at $\approx 100$ km/s. The density profile of the jet corresponds to a dense shell surrounding a low-density core, which is consistent with the centrifugal barrier effect being sustained along the jet's propagation. We show analytically that, as the rotating plasma accretes mass, conservation of mass and momentum implies plasma radial growth scaling as $r \propto t^{1/3}$. As the characteristic moment of inertia increases, the rotation velocity is predicted to decrease and settle on a characteristic value $\approx 20$ km/s. We find that both predictions are in agreement with Thomson scattering and optical self-emission imaging measurements.

==> jpp-bib.tex <==
% This is JPP2esam.bib v1.0 08/14/02
%

@book{J.FrankA.King2002,
address = {New York},
author = {J. Frank and A. King and D. Raine},
edition = {Third},
publisher = {Cambridge University Press},
title = {{Accretion power in astrophysics}},
year = {2002}
}


@article{Lesur2021,
author = {Lesur, Geoffroy R.J.},
doi = {10.1017/s0022377820001002},
eprint = {2007.15967},
issn = {23318422},
journal = {Journal of Plasma Physics},
keywords = {astrophysical plasmas,plasma instabilities},
pages = {205870101},
title = {{Magnetohydrodynamics of protoplanetary discs}},
volume = {87},
year = {2021}
}

@article{Lynden-Bell1996,
author = {Lynden-Bell, D.},
doi = {10.1093/mnras/279.2.389},
journal = {Monthly Notices of the Royal Astronomical Society},
keywords = {Accretion,Galaxies: jets,Magnetic fields,Quasars: general,Stars: activity,Stars: formation,accretion discs},
number = {2},
pages = {389--401},
title = {{Magnetic collimation by accretion discs of quasars and stars}},
volume = {279},
year = {1996}
}


@article{Shakura1973,
author = {Shakura, N. I. and Sunyaev, R. A.},
journal = {Astronomy \& Astrophysics},
pages = {337 -- 355},
title = {{Black holes in binary systems. Observational appearance}},
volume = {24},
year = {1973}
}

@book{Chandrasekhar1961,
author = {Chandrasekhar, S.},
edition = {First},
publisher = {Oxford University Press},
title = {{Hydrodynamic and hydromagnetic stability}},
year = {1961}
}

@article{Edlund2014,
author = {Edlund, E. M. and Ji, H.},
doi = {10.1103/PhysRevE.89.021004},
issn = {15393755},
journal = {Physical Review E - Statistical, Nonlinear, and Soft Matter Physics},
number = {2},
pages = {1--5},
title = {{Nonlinear stability of laboratory quasi-Keplerian flows}},
volume = {89},
year = {2014}
}


@article{Velikhov1959,
author = {Velikhov, E. P.},
issn = {1049-6491},
journal = {Soviet Physics JETP},
number = {5},
pages = {995},
title = {{Stability of an ideally conducting liquid flowing between cylinders rotating in a magnetic field}},
volume = {36},
year = {1959}
}


@article{Balbus1991,
author = {Balbus, S. A. and Hawley, J. F.},
journal = {The Astrophysical Journal},
pages = {214--222},
title = {{A powerful local shear instability in weakly magnetized disks}},
volume = {376},
year = {1991}
}

@article{Goodman1994,
author = {Goodman, J. and Xu, G.},
journal = {The Astrophysical Journal},
pages = {213 --223},
title = {{Parasitic instabilities in magnetized, differentially rotating disks}},
url = {http://iopscience.iop.org/0004-637X/644/1/651},
volume = {432},
year = {1994}
}

@article{Balbus1998,
author = {Balbus, Steven A and Hawley, John F},
doi = {10.1016/S0022-5347(17)36336-X},
journal = {Reviews of Modern Physics},
number = {5},
pages = {53},
title = {{Instability, turbulence, and enhanced transport in accretion disks}},
volume = {70},
year = {1998}
}


@article{Ji2006,
author = {Ji, H. and Burin, M. and Schartman, E. and Goodman, J.},
doi = {10.1038/nature05323},
isbn = {400,400,53,53},
issn = {14764687},
journal = {Nature},
number = {7117},
pages = {343--346},
pmid = {17108959},
title = {{Hydrodynamic turbulence cannot transport angular momentum effectively in astrophysical disks}},
volume = {444},
year = {2006}
}


@article{Ji2001,
author = {Ji, H. and Goodman, J. and Kageyama, A.},
doi = {10.1046/j.1365-8711.2001.04647.x},
issn = {00358711},
journal = {Monthly Notices of the Royal Astronomical Society},
keywords = {Accretion, accretion discs,Galaxy: disc,Instabilities,MHD,Magnetic fields,Planetary systems: protoplanetary discs},
number = {2},
pages = {L1--L5},
title = {{Magnetorotational instability in a rotating liquid metal annulus}},
volume = {325},
year = {2001}
}

@article{Ryutov1999,
author = {Ryutov, D. and Drake, R.P. and Kane, J. and Liang, E. and Remington, B. A. and Wood-Vasey, W. M.},
doi = {10.1088/0004-637X/698/2/2144},
isbn = {0004-637X},
issn = {15384357},
journal = {The Astrophysical Journal},
pages = {821 -- 832},
title = {{Similarity criteria for the laboratory simulation of supernova hydrodynamics}},
volume = {518},
year = {1999}
}

@article{Wang2022a,
author = {Wang, Yin and Gilson, Erik P. and Ebrahimi, Fatima and Goodman, Jeremy and Ji, Hantao},
doi = {10.1103/PhysRevLett.129.115001},
issn = {10797114},
journal = {Physical Review Letters},
keywords = {doi:10.1103/PhysRevLett.129.115001 url:https://doi},
number = {11},
pages = {115001},
pmid = {36154406},
publisher = {American Physical Society},
title = {{Observation of Axisymmetric Standard Magnetorotational Instability in the Laboratory}},
url = {https://doi.org/10.1103/PhysRevLett.129.115001},
volume = {129},
year = {2022}
}


@article{Wang2022b,
author = {Wang, Yin and Gilson, Erik P. and Ebrahimi, Fatima and Goodman, Jeremy and Caspary, Kyle J. and Winarto, Himawan W. and Ji, Hantao},
doi = {10.1038/s41467-022-32278-0},
isbn = {4146702232},
issn = {20411723},
journal = {Nature Communications},
number = {1},
pages = {1--10},
pmid = {35945242},
publisher = {Springer US},
title = {{Identification of a non-axisymmetric mode in laboratory experiments searching for standard magnetorotational instability}},
volume = {13},
year = {2022}
}


@article{Remington2006,
author = {Remington, Bruce A. and Drake, R. Paul and Ryutov, Dmitri D.},
doi = {10.1103/RevModPhys.78.755},
isbn = {0034-6861},
issn = {00346861},
journal = {Reviews of Modern Physics},
number = {3},
pages = {755--807},
title = {{Experimental astrophysics with high power lasers and Z pinches}},
volume = {78},
year = {2006}
}

@article{Takabe2021,
author = {Takabe, Hideaki and Kuramitsu, Yasuhiro},
doi = {10.1017/hpl.2021.35},
issn = {20523289},
journal = {High Power Laser Science and Engineering},
keywords = {Weibel instability,collisionless shock,compressible hydrodynamics,cosmic rays,equation of state,high-energy-density plasmas,intense laser,magnetic turbulence,opacity experiment,particle accelerations,relativistic plasmas,turbulent mixing,wakefield acceleration},
title = {{Recent progress of laboratory astrophysics with intense lasers}},
volume = {9},
year = {2021}
}




@article{Lebedev2019,
author = {Lebedev, S. V. and Frank, A. and Ryutov, D. D.},
doi = {10.1103/RevModPhys.91.025002},
issn = {0034-6861},
journal = {Reviews of Modern Physics},
keywords = {doi:10.1103/RevModPhys.91.025002 url:https://doi.o},
mendeley-groups = {PoP paper,PRL bibliography,00 THESIS BIB},
number = {2},
pages = {025002},
publisher = {American Physical Society},
title = {{Exploring astrophysics-relevant magnetohydrodynamics with pulsed-power laboratory facilities}},
url = {https://link.aps.org/doi/10.1103/RevModPhys.91.025002},
volume = {91},
year = {2019}
}

@article{Cvejic2022,
author = {Cveji{\'{c}}, M. and Mikitchuk, D. and Kroupp, E. and Doron, R. and Sharma, P. and Maron, Y. and Velikovich, A. L. and Fruchtman, A. and Ochs, I. E. and Kolmes, E. J. and Fisch, N. J.},
doi = {10.1103/PhysRevLett.128.015001},
journal = {Physical Review Letters},
pages = {015001},
title = {{Self-generated plasma rotation in a Z-pinch implosion with preembedded axial magnetic field}},
url = {http://arxiv.org/abs/2104.07342},
volume = {128},
year = {2022}
}

@article{Bocchi2013a,
author = {Bocchi, Matteo and Chittenden, Jerry P. and Lebedev, Sergey V. and Hall, Gareth N. and Bennett, Matthew and Frank, Adam and Blackman, Eric G.},
doi = {10.1016/j.hedp.2012.12.001},
isbn = {1574-1818},
issn = {15741818},
journal = {Astrophysical Journal},
pages = {84},
title = {{Numerical simulations of Z-pinch experiments to create supersonic differentially-rotating plasma flows}},
volume = {767},
year = {2013}
}


@article{Bocchi2013b,
author = {Bocchi, Matteo and Chittenden, Jerry P. and Lebedev, Sergey V. and Hall, Gareth N. and Bennett, Matthew and Frank, Adam and Blackman, Eric G.},
doi = {10.1016/j.hedp.2012.12.001},
issn = {15741818},
journal = {High Energy Density Physics},
mendeley-groups = {PRL bibliography,00 THESIS BIB},
number = {1},
pages = {108--111},
title = {{Numerical simulations of Z-pinch experiments to create supersonic differentially-rotating plasma flows}},
url = {http://dx.doi.org/10.1016/j.hedp.2012.12.001},
volume = {9},
year = {2013}
}


@article{Geyko2013,
author = {Geyko, V. I. and Fisch, N. J.},
doi = {10.1103/PhysRevLett.110.150604},
issn = {00319007},
journal = {Physical Review Letters},
number = {15},
pages = {1--5},
title = {{Reduced compressibility and an inverse problem for a spinning gas}},
volume = {110},
year = {2013}
}


@article{Geyko2017,
abstract = {A rotating plasma column is shown to exhibit unusual heat capacity effects under compression. For near equilibrium thermodynamics and smooth wall conditions, the heat capacity depends on the plasma density, on the speed of the rotation, and on the mass ratio. For a certain range of parameters, the storage of energy in the electric field produces a significant increase in the heat capacity.},
author = {Geyko, V. I. and Fisch, N. J.},
doi = {10.1063/1.4975651},
issn = {10897674},
journal = {Physics of Plasmas},
number = {2},
title = {{Compressibility and heat capacity of rotating plasma}},
url = {http://dx.doi.org/10.1063/1.4975651},
volume = {24},
year = {2017}
}


@article{Beresnyak2023,
author = {Beresnyak, Andrey and Velikovich, Alexander L. and Giuliani, John L. and Dasgupta, Arati},
doi = {10.1109/tps.2023.3340980},
issn = {0093-3813},
journal = {IEEE Transactions on Plasma Science},
number = {12},
pages = {1--7},
publisher = {IEEE},
title = {{Stable and Unstable Solutions of the Mag Noh Problem}},
volume = {51},
year = {2023}
}

@article{Benjamin1981,
author = {Benjamin, R. F. and Pearlman, J. S. and Chu, E. Y. and Riordan, J. C.},
doi = {10.1063/1.92581},
issn = {00036951},
journal = {Applied Physics Letters},
number = {10},
pages = {848--850},
title = {{Measurements of the dynamics of imploding wire arrays}},
volume = {39},
year = {1981}
}


@article{Aivazov1987,
author = {Aivazov, I. K. and Vikharev, V. D. and Volkov, G. S. and Nikandrov, L. B. and Smirnov, V. P. and Tsarfin, V. Ya.},
journal = {Journal of Experimental and Theoretical Physics Letters},
pages = {23},
title = {{Formation of a plasma precursor due to the collapse of mutiwire liners}},
volume = {1},
year = {1987}
}


@article{Aivazov1988,
author = {I. K. Aivazov and V. D. Vikharev and G. S. Volkov and L. B. Nikandrov and V. P. Smirnov and V. Ya. Tsarfi},
pages = {110},
journal = {Soviet Journal of Plasma Physics},
title = {{Study of exploding wire in high current accelerator}},
volume = {14},
year = {1988}
}

@article{Deeney1995,
author = {Deeney, C. and LePell, P. D. and Failor, B. H. and Wong, S. L. and Apruzese, J. P. and Whitney, K. G. and Thornhill, J. W. and Davis, J. and Yadlowsky, E. and Hazelton, R. C. and Moschella, J. J. and Nash, T. and Loter, N.},
number = {5},
pages = {4823},
title = {{Increased kilo-electron-volt x-ray yields from Z-pinch plasmas by mixing elements of similar atomic numbers}},
volume = {51},
year = {1995}
}

@article{Yadlowsky1996,
author = {Yadlowsky, E. J. and Moschella, J. J. and Hazelton, R. C. and Settersten, T. B. and Spanjers, G. G. and Deeney, C. and Failor, B. H. and LePell, P. D. and Davis, J. and Apruzese, J. P. and Whitney, K. G. and Thomhill, J. W.},
doi = {10.1063/1.871693},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {5},
pages = {1745--1753},
title = {{Evidence for precursor plasma formation resulting from heterogeneous current channels in wire arry loads}},
volume = {3},
year = {1996}
}




@article{Lebedev2000,
author = {Lebedev, S. V. and Beg, F. N. and Bland, S. N. and Chittenden, J. P. and Dangor, A. E. and Haines, M. G. and Pikuz, S. A. and Shelkovenko, T. A.},
doi = {10.1103/PhysRevLett.85.98},
journal = {Physical Review Letters},
number = {1},
pages = {98--101},
title = {{Effect of core-corona plasma structure on seeding of instabilities in wire array Z pinches}},
volume = {85},
year = {2000}
}

@phdthesis{Valenzuela-Villaseca2022,
author = {Valenzuela-Villaseca, Vicente},
doi = {10.25560/100847},
pages = {303},
school = {Imperial College London},
title = {{Experimental Study of Magneto-Inertially Driven , Differentially Rotating Plasma Flows}},
url = {http://hdl.handle.net/10044/1/100847},
year = {2022}
}


@article{Lebedev2005,
author = {Lebedev, S. V. and Ampleford, D. J. and Bland, S. N. and Bott, S. C. and Chittenden, J. P. and Goyer, J. and Jennings, C. and Haines, M. G. and Hall, G. N. and Hammer, D. A. and Palmer, J. B.A. and Pikuz, S. A. and Shelkovenko, T. A. and Christoudias, T.},
doi = {10.1088/0741-3335/47/5A/009},
issn = {07413335},
journal = {Plasma Physics and Controlled Fusion},
number = {5 A},
title = {{Physics of wire array Z-pinch implosions: Experiments at Imperial College}},
volume = {47},
year = {2005}
}

@article{Spielman1998,
author = {Spielman, R. B. and Deeney, C. and Chandler, G. A. and Douglas, M. R. and Fehl, D. L. and Matzen, M. K. and McDaniel, D. H. and Nash, T. J. and Porter, J. L. and Sanford, T. W. L. and Seamen, J. F. and Stygar, W. A. and Struve, K. W. and Breeze, S. P. and McGurn, J. S. and Torres, J. A. and Zagar, D. M. and Gilliland, T. L. and Jobe, D. O. and McKenney, J. L. and Mock, R. C. and Vargas, M. and Wagoner, T. and Peterson, D. L.},
doi = {10.1063/1.872881},
issn = {1070-664X},
journal = {Physics of Plasmas},
mendeley-groups = {00 THESIS BIB},
number = {5},
pages = {2105--2111},
title = {{Tungsten wire-array Z-pinch experiments at 200 TW and 2 MJ}},
volume = {5},
year = {1998}
}



@article{Harvey-Thompson2012a,
author = {Harvey-Thompson, A. J. and Lebedev, S. V. and Patankar, S. and Bland, S. N. and Burdiak, G. and Chittenden, J. P. and Colaitis, A. and {De Grouchy}, P. and Doyle, H. W. and Hall, G. N. and Khoory, E. and Hohenberger, M. and Pickworth, L. and Suzuki-Vidal, F. and Smith, R. A. and Skidmore, J. and Suttle, L. and Swadling, G. F.},
doi = {10.1103/PhysRevLett.108.145002},
journal = {Physical Review Letters},
number = {14},
pages = {145002},
title = {{Optical Thomson scattering measurements of plasma parameters in the ablation stage of wire array Z pinches}},
volume = {108},
year = {2012}
}

@article{Harvey-Thompson2012b,
author = {Harvey-Thompson, A. J. and Lebedev, S. V. and Patankar, S. and Bland, S. N. and Burdiak, G. and Chittenden, J. P. and Colaitis, A. and {De Grouchy}, P. and Hall, G. N. and Khoory, E. and Hohenberger, M. and Pickworth, L. and Suzuki-Vidal, F. and Smith, R. A. and Skidmore, J. and Suttle, L. and Swadling, G. F.},
doi = {10.1063/1.3694671},
journal = {Physics of Plasmas},
number = {5},
pages = {056303},
title = {{Optical Thomson scattering measurements of cylindrical wire array parameters}},
volume = {19},
year = {2012}
}



@article{Goodman2002,
author = {Goodman, J. and Ji, H.},
doi = {10.1017/S0022112002008704},
issn = {00221120},
journal = {Journal of Fluid Mechanics},
pages = {365--382},
title = {{Magnetorotational instability of dissipative Couette flow}},
volume = {462},
year = {2002}
}


@article{Hollerbach2005,
author = {Hollerbach, R. and R{\"{u}}diger, G.},
doi = {10.1103/PhysRevLett.95.124501},
issn = {00319007},
journal = {Physical Review Letters},
number = {12},
pages = {124501},
title = {{New type of magnetorotational instability in cylindrical Taylor-couette flow}},
volume = {95},
year = {2005}
}

@book{Hutchinson2002,
    author = {I. H. Hutchinson},
    title = {{Principles of Plasma Diagnostics}},
    publisher = {Cambridge University Press},
    year = {2002}
}

@book{Froula2011,
author = {Froula, D. and Glenzer, S. H. and Luhmann Jr., N. C. and Sheffield, J.},
title = {{Plasma scattering of electromagnetic radiation: theory and measurement techniques (2nd Edition)}},
publisher = {Elsevier},
year = {2011}
}

@phdthesis{Hare2017Thesis,
    author = {Hare, Jack Davies},
    title = {{High Energy Density Magnetic Reconnection Experiments in Colliding Carbon Plasma Flows}},
    school = {Imperial College London},
    year = {2017} 
}


@article{Stefani2006,
author = {Stefani, F. and Gundrum, T. and Gerbeth, G. and R{\"{u}}diger, G. and Schultz, M. and Szklarski, J. and Hollerbach, R.},
doi = {10.1103/PhysRevLett.97.184502},
issn = {00319007},
journal = {Physical Review Letters},
number = {18},
pages = {184502},
pmid = {17155546},
title = {{Experimental evidence for magnetorotational instability in a Taylor-Couette flow under the influence of a helical magnetic field}},
volume = {97},
year = {2006}
}

@article{Liu2006,
author = {Liu, W. and Goodman, J. and Herron, I. and Ji, H.},
doi = {10.1103/PhysRevE.76.068301},
isbn = {18650929 (ISSN); 9783319952031 (ISBN)},
issn = {15393755},
journal = {Physical Review E - Statistical, Nonlinear, and Soft Matter Physics},
pages = {056302},
title = {{Helical magnetorotational instability in magnetized Taylor-Couette flow}},
volume = {74},
year = {2006}
}

@article{Collins2012,
author = {Collins, C. and Katz, N. and Wallace, J. and Jara-Almonte, J. and Reese, I. and Zweibel, E. and Forest, C. B.},
doi = {10.1103/PhysRevLett.108.115001},
issn = {00319007},
journal = {Physical Review Letters},
mendeley-groups = {PRL bibliography},
number = {11},
pages = {115001},
title = {{Stirring unmagnetized plasma}},
volume = {108},
year = {2012}
}

@article{Flanagan2020,
author = {Flanagan, K. and Milhone, J. and Egedal, J. and Endrizzi, D. and Olson, J. and Peterson, E. E. and Sassella, R. and Forest, C. B.},
doi = {10.1103/physrevlett.125.135001},
issn = {0031-9007},
journal = {Physical Review Letters},
keywords = {doi:10.1103/PhysRevLett.125.135001 url:https://doi},
number = {13},
pages = {135001},
publisher = {American Physical Society},
title = {{Weakly magnetized, Hall dominated plasma Couette flow}},
url = {https://doi.org/10.1103/PhysRevLett.125.135001},
volume = {125},
year = {2020}
}

@article{Milhone2021,
author = {Milhone, J. and Flanagan, K. and Egedal, J. and Endrizzi, D. and Olson, J. and Peterson, E. E. and Wright, J. C. and Forest, C. B.},
doi = {10.1103/PhysRevLett.126.185002},
issn = {10797114},
journal = {Physical Review Letters},
keywords = {doi:10.1103/PhysRevLett.126.185002 url:https://doi},
number = {18},
pages = {185002},
publisher = {American Physical Society},
title = {{Ion heating and flow driven by an instability found in plasma Couette flow}},
url = {https://doi.org/10.1103/PhysRevLett.126.185002},
volume = {126},
year = {2021}
}

@article{Blandford1982,
author = {Blandford, R. D. and Payne, D. G.},
journal = {Monthly Notices of the Royal Astronomical Society},
number = {4},
pages = {883},
title = {{Hydromagnetic flows from accretion discs and the production of radio jets}},
volume = {199},
year = {1982}
}


@article{Begelman1984,
author = {Begelman, M. C. and Blandford, R. D. and Rees, M. J.},
doi = {10.1103/RevModPhys.56.255},
issn = {00346861},
journal = {Reviews of Modern Physics},
number = {2},
pages = {255--351},
title = {{Theory of extragalactic radio sources}},
volume = {56},
year = {1984}
}

@article{Reipurth2001,
author = {Reipurth, Bo and Bally, John},
journal = {Annular review of Astronomy and Astrophysics},
pages = {403},
title = {{Herbig-Haro flows: probes of early stellar evolution}},
volume = {39},
year = {2001}
}

@article{Coffey2004,
author = {Coffey, D. and Bacciotti, F. and Woitas, J. and Ray, T. P. and Eislo, J.},
journal = {The Astrophysical Journal},
pages = {758--765},
title = {{Rotation of Jets From Young Stars : New Clues From the Hubble}},
volume = {604},
year = {2004}
}





@article{Matsushita2021,
author = {Matsushita, Y. and Takahashi, S. and Ishii, S. and Tomisaka, K. and Ho, P. T. P. and Carpenter, J. M. and Machida, M. N.},
doi = {10.3847/1538-4357/ac069f},
eprint = {2107.12002},
issn = {0004-637X},
journal = {The Astrophysical Journal},
keywords = {Star formation,Stellar jets,Stellar winds},
number = {1},
pages = {23},
publisher = {IOP Publishing},
title = {{Super-fast Rotation in the OMC 2/FIR 6b Jet}},
url = {http://dx.doi.org/10.3847/1538-4357/ac069f},
volume = {916},
year = {2021}
}

@article{Narayan2005,
author = {Narayan, Ramesh and Quataert, Eliot},
doi = {10.1126/science.1105746},
issn = {00368075},
journal = {Science},
number = {5706},
pages = {77--80},
title = {{Black hole accretion}},
volume = {307},
year = {2005}
}


@article{Pringle1981,
author = {Pringle, J. E.},
journal = {Annual review of Astronomy and Astrophysics},
pages = {137--163},
title = {{Accretion discs in astrophysics}},
url = {https://doi.org/10.1146/annurev.aa.19.090181.001033},
volume = {19},
year = {1981}
}


@article{Gissinger2011,
author = {Gissinger, C. and Ji, H. and Goodman, J.},
doi = {10.1103/PhysRevE.84.026308},
issn = {15393755},
journal = {Physical Review E - Statistical, Nonlinear, and Soft Matter Physics},
number = {2},
pages = {026308},
title = {{Instabilities in magnetized spherical Couette flow}},
volume = {84},
year = {2011}
}

@article{Edlund2015,
author = {Edlund, E. M. and Ji, H.},
doi = {10.1103/PhysRevE.92.043005},
issn = {15502376},
journal = {Physical Review E - Statistical, Nonlinear, and Soft Matter Physics},
number = {4},
pages = {043005},
title = {{Reynolds number scaling of the influence of boundary layers on the global behavior of laboratory quasi-Keplerian flows}},
volume = {92},
year = {2015}
}


@article{Mitchell1996,
author = {Mitchell, I H and Bayley, J M and Chittenden, J P and Worley, J F and Dangor, a E and Haines, M G and Choi, P},
doi = {Doi 10.1063/1.1146884},
isbn = {0034-6748},
issn = {00346748},
journal = {Review of Scientific Instruments},
keywords = {radiative collapse},
number = {4},
pages = {1533--1541},
title = {{A high impedance mega-ampere generator for fiber z-pinch experiments}},
volume = {67},
year = {1996}
}

@article{Lebedev2001a,
author = {Lebedev, S. V. and Beg, F. N. and Bland, S. N. and Chittenden, J. P. and Dangor, A. E. and Haines, M. G. and Pikuz, S. A. and Shelkovenko, T. A.},
doi = {10.1017/S0263034601193122},
issn = {02630346},
journal = {Laser and Particle Beams},
number = {3},
pages = {355--376},
publisher = {Imperial College London Library},
title = {{Plasma formation and the implosion phase of wire array z-pinch experiments}},
volume = {19},
year = {2001}
}

@article{Bott2006,
author = {Bott, S. C. and Lebedev, S. V. and Ampleford, D. J. and Bland, S. N. and Chittenden, J. P. and Ciardi, A. and Haines, M. G. and Jennings, C. and Sherlock, M. and Hall, G. and Rapley, J. and Beg, F. N. and Palmer, J.},
doi = {10.1103/PhysRevE.74.046403},
issn = {15393755},
journal = {Physical Review E - Statistical, Nonlinear, and Soft Matter Physics},
mendeley-groups = {PRL bibliography},
number = {4},
pages = {046403},
pmid = {17155178},
title = {{Dynamics of cylindrically converging precursor plasma flow in wire-array Z -pinch experiments}},
volume = {74},
year = {2006}
}

@article{Bennett2015,
abstract = {We present data from the first Z-pinch experiments aiming to simulate aspects of accretion disk physics in the laboratory. Using off axis ablation flows from a wire array z-pinch we demonstrate the formation of a supersonically (M $\sim$ 2) rotating hollow plasma cylinder of height $\sim$4mm and radius 2 mm. Using a combination of diagnostics we measure the rotation speed ($\sim$60kms-1), electron density (1019cm-3), ion temperature (Ti $\sim$ 60eV) and the product of electron temperature and average ionisation (ZTe $\sim$ 150 to 200 eV). Using these parameters we calculate the Reynolds number for the plasma on the order 105 and magnetic Reynolds number as 10 - 100. The plasma flow is maintained for 150ns, corresponding to one rotation period, which should allow for studying fast instabilities which develop on this time-scale.},
author = {Bennett, M. J. and Lebedev, S. V. and Hall, G. N. and Suttle, L. and Burdiak, G. and Suzuki-Vidal, F. and Hare, J. and Swadling, G. and Patankar, S. and Bocchi, M. and Chittenden, J. P. and Smith, R. and Frank, A. and Blackman, E. and Drake, R. P. and Ciardi, A.},
doi = {10.1016/j.hedp.2015.02.001},
file = {:C\:/Users/valen/Documents/PAPERS/Formation of radiatively cooled, supersonically rotating, plasma flows in Z pinch experiments.pdf:pdf},
issn = {15741818},
journal = {High Energy Density Physics},
keywords = {Accretion disks,High energy density,Laboratory astrophysics,Rotating plasma,Supersonic flow},
mendeley-groups = {NIF proposal 2019,PoP paper,PRL bibliography,00 THESIS BIB,ApJ paper,NLUF FY2024,JPP bib},
pages = {63--67},
publisher = {Elsevier},
title = {{Formation of radiatively cooled, supersonically rotating, plasma flows in Z-pinch experiments: Towards the development of an experimental platform to study accretion disk physics in the laboratory}},
volume = {17},
year = {2015}
}



@article{Swadling2013,
author = {Swadling, G. F. and Lebedev, S. V. and Niasse, N. and Chittenden, J. P. and Hall, G. N. and Suzuki-Vidal, F. and Burdiak, G. and Harvey-Thompson, A. J. and Bland, S. N. and {De Grouchy}, P. and Khoory, E. and Pickworth, L. and Skidmore, J. and Suttle, L.},
doi = {10.1063/1.4790520},
issn = {1070664X},
journal = {Physics of Plasmas},
number = {2},
pages = {022705},
title = {{Oblique shock structures formed during the ablation phase of aluminium wire array z-pinches}},
volume = {20},
year = {2013}
}

@article{Hare2019,
author = {Hare, J D and MacDonald, J and Bland, S N and Dranczewski, J and Halliday, J W D and Lebedev, S V and Suttle, L G and Tubman, E R and Rozmus, W},
doi = {10.1088/1361-6587/ab2571},
issn = {0741-3335},
journal = {Plasma Physics and Controlled Fusion},
number = {8},
pages = {085012},
publisher = {IOP Publishing},
title = {{Two-colour interferometry and Thomson scattering measurements of a plasma gun}},
volume = {61},
year = {2019}
}



@article{Swadling2014,
author = {Swadling, G. F. and Lebedev, S. V. and Hall, G. N. and Patankar, S. and Stewart, N. H. and Smith, R. A. and Harvey-Thompson, A. J. and Burdiak, G. C. and {De Grouchy}, P. and Skidmore, J. and Suttle, L. and Suzuki-Vidal, F. and Bland, S. N. and Kwek, K. H. and Pickworth, L. and Bennett, M. and Hare, J. D. and Rozmus, W. and Yuan, J.},
doi = {10.1063/1.4890564},
isbn = {1089-7623 (Electronic)
0034-6748 (Linking)},
issn = {10897623},
journal = {Review of Scientific Instruments},
number = {11},
pmid = {25430344},
title = {{Diagnosing collisions of magnetized, high energy density plasma flows using a combination of collective Thomson scattering, Faraday rotation, and interferometry (invited)}},
volume = {85},
year = {2014}
}

@article{Ampleford2008,
abstract = {The first laboratory astrophysics experiments to produce a radiatively cooled plasma jet with dynamically significant angular momentum are discussed. A new configuration of wire array z pinch, the twisted conical wire array, is used to produce convergent plasma flows each rotating about the central axis. Collision of the flows produces a standing shock and jet that each have supersonic azimuthal velocities. By varying the twist angle of the array, the rotation velocity of the system can be controlled, with jet rotation velocities reaching approximately 18% of the propagation velocity.},
author = {Ampleford, D. J. and Lebedev, S. V. and Ciardi, A. and Bland, S. N. and Bott, S. C. and Hall, G. N. and Naz, N. and Jennings, C. A. and Sherlock, M. and Chittenden, J. P. and Palmer, J. B A and Frank, A. and Blackman, E.},
doi = {https://doi.org/10.1103/PhysRevLett.100.035001},
file = {:C\:/Users/valen/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Ampleford et al. - 2008 - Supersonic radiatively cooled rotating flows and jets in the laboratory.pdf:pdf},
journal = {Physical Review Letters},
mendeley-groups = {PRL bibliography,00 THESIS BIB,JPP bib},
number = {3},
pages = {1--4},
title = {{Supersonic radiatively cooled rotating flows and jets in the laboratory}},
volume = {100},
year = {2008}
}




@article{Valenzuela-Villaseca2023,
abstract = {We present results from pulsed-power driven differentially rotating plasma experiments designed to simulate physics relevant to astrophysical disks and jets. In these experiments, angular momentum is injected by the ram pressure of the ablation flows from a wire array Z pinch. In contrast to previous liquid metal and plasma experiments, rotation is not driven by boundary forces. Axial pressure gradients launch a rotating plasma jet upwards, which is confined by a combination of ram, thermal, and magnetic pressure of a surrounding plasma halo. The jet has subsonic rotation, with a maximum rotation velocity $23 \pm 3$ km/s. The rotational velocity profile is quasi-Keplerian with a positive Rayleigh discriminant $\kappa^2 \propto r^{-2.8\pm0.8}$ rad$^2$/s$^2$. The plasma completes $0.5 - 2$ full rotations in the experimental time frame ($\sim 150$ ns).},
archivePrefix = {arXiv},
arxivId = {2201.10339},
author = {Valenzuela-Villaseca, V. and Suttle, L. G. and Suzuki-Vidal, F. and Halliday, J. W. D. and Merlini, S. and Russell, D. R. and Tubman, E. R. and Hare, J. D. and Chittenden, J. P. and Koepke, M. E. and Blackman, E. G. and Lebedev, S. V.},
doi = {10.1103/PhysRevLett.130.195101},
eprint = {2201.10339},
file = {:C\:/Users/valen/Documents/PAPERS/Characterization of quasi Keplerian, differentially rotating, free boundary laboratory plasmas.pdf:pdf},
issn = {1079-7114},
journal = {Physical Review Letters},
keywords = {doi:10.1103/PhysRevLett.130.195101 url:https://doi},
mendeley-groups = {IEEE paper},
number = {19},
pages = {195101},
publisher = {American Physical Society},
title = {{Characterization of Quasi-Keplerian, Differentially Rotating, Free-Boundary Laboratory Plasmas}},
url = {http://arxiv.org/abs/2201.10339},
volume = {130},
year = {2023}
}

@article{Felber1981,
author = {Felber, F. S. and Rostoker, N.},
doi = {10.1192/bjp.112.483.211-a},
file = {:C\:/Users/valen/Documents/PAPERS/Kink and displacement instabilities in imploding wire arrays.pdf:pdf},
issn = {0007-1250},
journal = {Physics of Fluids},
keywords = {behaviour therapy,clinical psychology,psychology},
mendeley-groups = {PoP paper,00 THESIS BIB,JPP bib},
number = {6},
pages = {1049},
title = {{Kind and displacement instabilities in imploding wire arrays}},
volume = {24},
year = {1981}
}


@article{Suttle2021,
author = {Suttle, L. G. and Hare, J. D. and Halliday, J. W.D. and Merlini, S. and Russell, D. R. and Tubman, E. R. and Valenzuela-Villaseca, V. and Rozmus, W. and Bruulsema, C. and Lebedev, S. V.},
doi = {10.1063/5.0041118},
file = {:C\:/Users/valen/Documents/PAPERS/Collective optical TS in pulsed power driven HEDP experiments.pdf:pdf},
journal = {Review of Scientific Instruments},
mendeley-groups = {PRL bibliography,00 THESIS BIB,JPP bib},
number = {3},
pages = {033542},
publisher = {AIP Publishing, LLC},
title = {{Collective optical Thomson scattering in pulsed-power driven high energy density physics experiments (invited)}},
url = {https://doi.org/10.1063/5.0041118},
volume = {92},
year = {2021}
}

@article{Dasch1992,
author = {Dasch, Cameron J.},
doi = {10.1364/ao.31.001146},
issn = {0003-6935},
journal = {Applied Optics},
number = {8},
pages = {1146},
pmid = {20720732},
title = {{One-dimensional tomography: a comparison of Abel, Dasch, C. J. (1992). One-dimensional tomography: a comparison of Abel, onion-peeling, and filtered backprojection methods. Applied Optics, 31(8), 1146. https://doi.org/10.1364/ao.31.001146onion-peeling, an}},
volume = {31},
year = {1992}
}

@article{Crilly2023,
author = {Crilly, A. J. and Niasse, N. P.L. and Fraser, A. R. and Chapman, D. A. and McLean, K. W. and Rose, S. J. and Chittenden, J. P.},
doi = {10.1016/j.hedp.2023.101053},
issn = {15741818},
journal = {High Energy Density Physics},
number = {November 2022},
pages = {101053},
publisher = {Elsevier B.V.},
title = {{SpK: A fast atomic and microphysics code for the high-energy-density regime}},
url = {https://doi.org/10.1016/j.hedp.2023.101053},
volume = {48},
year = {2023}
}


@article{Balbus2008,
author = {Balbus, Steven A. and Henri, Pierre},
doi = {10.1086/524838},
journal = {The Astrophysical Journal},
number = {1},
pages = {408--414},
title = {{On the Magnetic Prandtl Number Behavior of Accretion Disks}},
volume = {674},
year = {2008}
}

@article{Schekochihin2004,
author = {Schekochihin, Alexander A. and Cowley, Steven C. and Maron, Jason L. and McWilliams, James C.},
doi = {10.1103/PhysRevLett.92.054502},
journal = {Physical Review Letters},
number = {5},
pages = {4},
title = {{Critical Magnetic Prandtl Number for Small-Scale Dynamo}},
volume = {92},
year = {2004}
}

@unpublished{Valenzuela-Villaseca2023b,
archivePrefix = {arXiv},
arxivId = {2312.02346},
author = {Valenzuela-Villaseca, V. and Suttle, L. G. and Suzuki-Vidal, F. and Halliday, J. W. D. and Russell, D. R. and Merlini, S. and Tubman, E. R. and Hare, J. D. and Chittenden, J. P. and Koepke, M. E. and Blackman, E. G. and Lebedev, S. V.},
eprint = {2312.02346},
file = {:C\:/Users/valen/Documents/PAPERS/On the structure of plasma jets in the rotating plasma experiment.pdf:pdf},
number = {8},
pages = {1--8},
title = {{On The Structure of Plasma Jets in the Rotating Plasma Experiment}},
url = {http://arxiv.org/abs/2312.02346},
volume = {14},
year = {2023}
}





%% End of file `JPP2esam.bib'.

